Transverse and spatial structure of light to heavy pseudoscalar mesons in light-cone quark model

In this work, we have investigated the transverse and spatial structure of light ($\pi^+ (u\bar d)$, $K^+(u\bar s)$) and heavy ($\eta_c(c\bar c)$, $\eta_b (b\bar b)$, $B$ and $D$) pseudoscalar mesons using the light-cone quark model. The transverse structure of these particles have been studied using the transverse momentum dependent parton distribution (TMDs). The leading twist unpolarized $f_1(x, \mathbf{k}_\perp^2)$ TMD has been solved using the quark-quark correlator. We have predicted the average momenta carried by the quark and antiquark of the considered mesons. For a complete description of mesons, we have also computed the leading twist unpolarized $H(x,0,-t)$ generalized parton distribution (GPD). Further, electromagnetic form factors (EMFFs), along with gravitational form factors (GFFs) have been derived by taking the zeroth and first moments of the unpolarized GPD. These EMFFs are found to be compatible with available lattice simulation results. Further, we have also calculated the parton distribution functions (PDFs) for both the quarks and the antiquarks of these mesons. The PDF sum rule has also been verified.

==> ref.tex <==
\bibitem{Lepage:1980fj}Lepage, G. \& Brodsky, S. Exclusive Processes in Perturbative Quantum Chromodynamics. {\em Phys. Rev. D}. \textbf{22} pp. 2157 (1980)
\bibitem{Brodsky:1997de}Brodsky, S., Pauli, H. \& Pinsky, S. Quantum chromodynamics and other field theories on the light cone. {\em Phys. Rept.}. \textbf{301} pp. 299-486 (1998)
\bibitem{Pasquini:2023aaf}Pasquini, B., Rodini, S. \& Venturini, S. Valence quark, sea, and gluon content of the pion from the parton distribution functions and the electromagnetic form factor. {\em Phys. Rev. D}. \textbf{107}, 114023 (2023)
\bibitem{Shi:2022erw}Shi, C., Li, J., Li, M., Chen, X. \& Jia, W. Transverse momentum distributions of valence quarks in light and heavy vector mesons. {\em Phys. Rev. D}. \textbf{106}, 014026 (2022)
\bibitem{Puhan_2024}Puhan, S. \& Dahiya, H. Spatial and Transverse structure of Heavy B- and D-mesons. {\em Proceedings Of 16th International Conference On Heavy Quarks And Leptons — PoS(HQL2023)}. pp. 089 (2024,4)
\bibitem{Qian:2008px}Qian, W. \& Ma, B. Vector meson omega-phi mixing and their form factors in light-cone quark model. {\em Phys. Rev. D}. \textbf{78} pp. 074002 (2008)
\bibitem{Xiao:2002iv}Xiao, B., Qian, X. \& Ma, B. The Kaon form-factor in the light cone quark model. {\em Eur. Phys. J. A}. \textbf{15} pp. 523-527 (2002)
\bibitem{Kaur:2020vkq}Kaur, S., Kumar, N., Lan, J., Mondal, C. \& Dahiya, H. Tomography of light mesons in the light-cone quark model. {\em Phys. Rev. D}. \textbf{102}, 014021 (2020)
\bibitem{Ma:1993ht}Ma, B. Spin structure of the pion in a light cone representation. {\em Z. Phys. A}. \textbf{345} pp. 321-325 (1993)
\bibitem{Yu:2007hp}Yu, J., Xiao, B. \& Ma, B. Space-like and time-like pion-rho transition form factors in the light-cone formalism. {\em J. Phys. G}. \textbf{34} pp. 1845-1860 (2007)
\bibitem{Arifi:2022pal}Arifi, A., Choi, H., Ji, C. \& Oh, Y. Mixing effects on 1S and 2S state heavy mesons in the light-front quark model. {\em Phys. Rev. D}. \textbf{106}, 014009 (2022)
\bibitem{Choi:1996mq}Choi, H. \& Ji, C. Light cone quark model predictions for radiative meson decays. {\em Nucl. Phys. A}. \textbf{618} pp. 291-316 (1997)
\bibitem{Diehl:2003ny}Diehl, M. Generalized parton distributions. {\em Phys. Rept.}. \textbf{388} pp. 41-277 (2003)
\bibitem{Bacchetta:2020vty}Bacchetta, A., Celiberto, F., Radici, M. \& Taels, P. Transverse-momentum-dependent gluon distribution functions in a spectator model. {\em Eur. Phys. J. C}. \textbf{80}, 733 (2020)
\bibitem{Kaur:2019jfa}Kaur, N. \& Dahiya, H. Transverse momentum dependent parton distributions of pion in the light-front holographic model. {\em Int. J. Mod. Phys. A}. \textbf{36}, 2150052 (2021)
\bibitem{Serna:2024vpn}Serna, F., El-Bennich, B. \& Krein, G. Parton distribution functions and transverse momentum dependence of heavy mesons.  (2024,9)
\bibitem{Almeida-Zamora:2023bqb}Almeida-Zamora, B., Cobos-Martı́nez, J., Bashir, A., Raya, K., Rodrı́guez-Quintero, J. \& Segovia, J. Algebraic model to study the internal structure of pseudoscalar mesons with heavy-light quark content. {\em Phys. Rev. D}. \textbf{109}, 014016 (2024)
\bibitem{Shi:2024laj}Shi, C., Liu, P., Du, Y. \& Jia, W. Heavy flavor-asymmetric pseudoscalar mesons on the light front.  (2024,9)
\bibitem{Lorce:2016ugb}Lorcé, C., Pasquini, B. \& Schweitzer, P. Transverse pion structure beyond leading twist in constituent models. {\em Eur. Phys. J. C}. \textbf{76}, 415 (2016)
\bibitem{Lorce:2014hxa}Lorcé, C., Pasquini, B. \& Schweitzer, P. Unpolarized transverse momentum dependent parton distribution functions beyond leading twist in quark models. {\em JHEP}. \textbf{1} pp. 103 (2015)
\bibitem{Albino:2022gzs}Albino, L., Higuera-Angulo, I., Raya, K. \& Bashir, A. Pseudoscalar mesons: Light front wave functions, GPDs, and PDFs. {\em Phys. Rev. D}. \textbf{106}, 034003 (2022)
\bibitem{Puhan2023}Puhan, S., Sharma, S., Kaur, N., Kumar, N. \& Dahiya, H. T-even TMDs for the spin-0 pseudo-scalar mesons upto twist-4 using light-front formalism. {\em JHEP}. \textbf{2} pp. 075 (2024)
\bibitem{Zhu:2023lst}Zhu, Z., Hu, Z., Lan, J., Mondal, C., Zhao, X. \& Vary, J. Transverse structure of the pion beyond leading twist with basis light-front quantization. {\em Phys. Lett. B}. \textbf{839} pp. 137808 (2023)
\bibitem{Aicher:2010cb}Aicher, M., Schafer, A. \& Vogelsang, W. Soft-gluon resummation and the valence parton distribution function of the pion. {\em Phys. Rev. Lett.}. \textbf{105} pp. 252003 (2010)
\bibitem{Lan:2019rba}Lan, J., Mondal, C., Jia, S., Zhao, X. \& Vary, J. Pion and kaon parton distribution functions from basis light front quantization and QCD evolution. {\em Phys. Rev. D}. \textbf{101}, 034024 (2020)
\bibitem{Cui:2020tdf}Cui, Z., Ding, M., Gao, F., Raya, K., Binosi, D., Chang, L., Roberts, C., Rodrı́guez-Quintero, J. \& Schmidt, S. Kaon and pion parton distributions. {\em Eur. Phys. J. C}. \textbf{80}, 1064 (2020)
\bibitem{Miyama:1995bd}Miyama, M. \& Kumano, S. Numerical solution of Q**2 evolution equations in a brute force method. {\em Comput. Phys. Commun.}. \textbf{94} pp. 185-215 (1996)
\bibitem{Hirai:1997gb}Hirai, M., Kumano, S. \& Miyama, M. Numerical solution of Q**2 evolution equations for polarized structure functions. {\em Comput. Phys. Commun.}. \textbf{108} pp. 38 (1998)
\bibitem{Hirai:1997mm}Hirai, M., Kumano, S. \& Miyama, M. Numerical solution of Q**2 evolution equation for the transversity distribution Delta(T)q. {\em Comput. Phys. Commun.}. \textbf{111} pp. 150-166 (1998)
\bibitem{Hirai:2011si}Hirai, M. \& Kumano, S. Numerical solution of Q² evolution equations for fragmentation functions. {\em Comput. Phys. Commun.}. \textbf{183} pp. 1002-1013 (2012)
\bibitem{Bourrely:2023yzi}Bourrely, C., Buccella, F., Chang, W. \& Peng, J. Extraction of kaon partonic distribution functions from Drell-Yan and J/\ensuremathψ production data. {\em Phys. Lett. B}. \textbf{848} pp. 138395 (2024)
\bibitem{Han:2020vjp}Han, C., Xie, G., Wang, R. \& Chen, X. An Analysis of Parton Distribution Functions of the Pion and the Kaon with the Maximum Entropy Input. {\em Eur. Phys. J. C}. \textbf{81}, 302 (2021)
\bibitem{Bednar:2018mtf}Bednar, K., Cloët, I. \& Tandy, P. Distinguishing Quarks and Gluons in Pion and Kaon Parton Distribution Functions. {\em Phys. Rev. Lett.}. \textbf{124}, 042002 (2020)
\bibitem{Brodsky:2007fr}Brodsky, S., Llanes-Estrada, F. \& Szczepaniak, A. Illuminating the 1/x moment of parton distribution functions. {\em EConf}. \textbf{C070910} pp. 149 (2007)
\bibitem{Brodsky:2000xy}Brodsky, S., Diehl, M. \& Hwang, D. Light cone wave function representation of deeply virtual Compton scattering. {\em Nucl. Phys. B}. \textbf{596} pp. 99-124 (2001)
\bibitem{Zhang:1997dd}Zhang, W. A Weak coupling treatment of nonperturbative QCD dynamics to heavy hadrons. {\em Phys. Rev. D}. \textbf{56} pp. 1528-1548 (1997)
\bibitem{Collins:1981uw}Collins, J. \& Soper, D. Parton Distribution and Decay Functions. {\em Nucl. Phys. B}. \textbf{194} pp. 445-492 (1982)
\bibitem{Martin:1998sq}Martin, A., Roberts, R., Stirling, W. \& Thorne, R. Parton distributions: A New global analysis. {\em Eur. Phys. J. C}. \textbf{4} pp. 463-496 (1998)
\bibitem{Gluck:1994uf}Gluck, M., Reya, E. \& Vogt, A. Dynamical parton distributions of the proton and small x physics. {\em Z. Phys. C}. \textbf{67} pp. 433-448 (1995)
\bibitem{Alekhin:2002fv}Alekhin, S. Parton distributions from deep inelastic scattering data. {\em Phys. Rev. D}. \textbf{68} pp. 014002 (2003)
\bibitem{Polchinski:2002jw}Polchinski, J. \& Strassler, M. Deep inelastic scattering and gauge / string duality. {\em JHEP}. \textbf{5} pp. 012 (2003)
\bibitem{Can:2012tx}Can, K., Erkol, G., Oka, M., Ozpineci, A. \& Takahashi, T. Vector and axial-vector couplings of D and D* mesons in 2+1 flavor Lattice QCD. {\em Phys. Lett. B}. \textbf{719} pp. 103-109 (2013)
\bibitem{NA7:1986vav}Amendolia, S. \& Others A Measurement of the Space - Like Pion Electromagnetic Form-Factor. {\em Nucl. Phys. B}. \textbf{277} pp. 168 (1986)
\bibitem{Dally:1982zk}Dally, E. \& Others Elastic Scattering Measurement of the Negative Pion Radius. {\em Phys. Rev. Lett.}. \textbf{48} pp. 375-378 (1982)
\bibitem{QCDSFUKQCD:2006gmg}Brömmel, D. \& Others The Pion form-factor from lattice QCD with two dynamical flavours. {\em Eur. Phys. J. C}. \textbf{51} pp. 335-345 (2007)
\bibitem{JeffersonLabFpi:2000nlc}Volmer, J. \& Others Measurement of the Charged Pion Electromagnetic Form-Factor. {\em Phys. Rev. Lett.}. \textbf{86} pp. 1713-1716 (2001)
\bibitem{JeffersonLabFpi-2:2006ysh}Horn, T. \& Others Determination of the Charged Pion Form Factor at Q**2 = 1.60 and 2.45-(GeV/c)**2. {\em Phys. Rev. Lett.}. \textbf{97} pp. 192001 (2006)
\bibitem{JeffersonLabFpi:2007vir}Tadevosyan, V. \& Others Determination of the pion charge form-factor for Q**2 = 0.60-GeV**2 - 1.60-GeV**2. {\em Phys. Rev. C}. \textbf{75} pp. 055205 (2007)
\bibitem{Dally:1980dj}Dally, E. \& Others DIRECT MEASUREMENT OF THE NEGATIVE KAON FORM-FACTOR. {\em Phys. Rev. Lett.}. \textbf{45} pp. 232-235 (1980)
\bibitem{Dias:2010sg}Dias, O., Filho, V. \& Melo, J. Kaon and Pion Electromagnetic Form Factor Ratios in the Light-Front. {\em Nucl. Phys. B Proc. Suppl.}. \textbf{199} pp. 281-284 (2010)
\bibitem{Amendolia:1986ui}Amendolia, S. \& Others A Measurement of the Kaon Charge Radius. {\em Phys. Lett. B}. \textbf{178} pp. 435-440 (1986)
\bibitem{Li:2017eic}Li, N. \& Wu, Y. Lattice study of D and Dₚ meson form factors with twisted boundary conditions. {\em Eur. Phys. J. A}. \textbf{53}, 56 (2017)
\bibitem{Li:2020gau}Li, N., Liu, C. \& Wu, Y. Lattice study of form factors for charmonium. {\em Eur. Phys. J. A}. \textbf{56}, 242 (2020)
\bibitem{Diehl:2015uka}Diehl, M. Introduction to GPDs and TMDs. {\em Eur. Phys. J. A}. \textbf{52}, 149 (2016)
\bibitem{Angeles-Martinez:2015sea}Angeles-Martinez, R. \& Others Transverse Momentum Dependent (TMD) parton distribution functions: status and prospects. {\em Acta Phys. Polon. B}. \textbf{46}, 2501-2534 (2015)
\bibitem{Pasquini:2008ax}Pasquini, B., Cazzaniga, S. \& Boffi, S. Transverse momentum dependent parton distributions in a light-cone quark model. {\em Phys. Rev. D}. \textbf{78} pp. 034025 (2008)
\bibitem{Chavez:2021llq}Chavez, J., Bertone, V., De Soto Borrero, F., Defurne, M., Mezrag, C., Moutarde, H., Rodrı́guez-Quintero, J. \& Segovia, J. Pion generalized parton distributions: A path toward phenomenology. {\em Phys. Rev. D}. \textbf{105}, 094012 (2022)
\bibitem{Zhang:2021tnr}Zhang, J. \& Ping, J. Kaon generalized parton distributions and light-front wave functions in the Nambu–Jona-Lasinio model. {\em Eur. Phys. J. C}. \textbf{81}, 814 (2021)
\bibitem{Broniowski:2022iip}Broniowski, W., Shastry, V. \& Ruiz Arriola, E. Off-shell generalized parton distributions and form factors of the pion. {\em Phys. Lett. B}. \textbf{840} pp. 137872 (2023)
\bibitem{Kaur:2023zhn}Kaur, N. \& Dahiya, H. Generalized parton distributions for the lowest-lying octet baryons. {\em Eur. Phys. J. A}. \textbf{60}, 42 (2024)
\bibitem{Guidal:2004nd}Guidal, M., Polyakov, M., Radyushkin, A. \& Vanderhaeghen, M. Nucleon form-factors from generalized parton distributions. {\em Phys. Rev. D}. \textbf{72} pp. 054013 (2005)
\bibitem{Kaur:2024wze}Kaur, N., Puhan, S., Pandey, R., Kumar, A., Dutt, S. \& Dahiya, H. Does nuclear medium affect the transverse momentum-dependent parton distributions of valence quark of pions?.  (2024,9)
\bibitem{Echevarria:2022ztg}Echevarria, M., Gutierrez Garcia, P. \& Scimemi, I. GTMDs and the factorization of exclusive double Drell-Yan. {\em Phys. Lett. B}. \textbf{840} pp. 137881 (2023)
\bibitem{Meissner:2009ww}Meissner, S., Metz, A. \& Schlegel, M. Generalized parton correlation functions for a spin-1/2 hadron. {\em JHEP}. \textbf{8} pp. 056 (2009)
\bibitem{Goeke:2005hb}Goeke, K., Metz, A. \& Schlegel, M. Parameterization of the quark-quark correlator of a spin-1/2 hadron. {\em Phys. Lett. B}. \textbf{618} pp. 90-96 (2005)
\bibitem{Bacchetta:2017gcc}Bacchetta, A., Delcarro, F., Pisano, C., Radici, M. \& Signori, A. Extraction of partonic transverse momentum distributions from semi-inclusive deep-inelastic scattering, Drell-Yan and Z-boson production. {\em JHEP}. \textbf{6} pp. 081 (2017), [Erratum: JHEP 06, 051 (2019)]
\bibitem{Makris:2020ltr}Makris, Y., Ringer, F. \& Waalewijn, W. Joint thrust and TMD resummation in electron-positron and electron-proton collisions. {\em JHEP}. \textbf{2} pp. 070 (2021)
\bibitem{Boer:1997mf}Boer, D., Jakob, R. \& Mulders, P. Asymmetries in polarized hadron production in e+ e- annihilation up to order 1/Q. {\em Nucl. Phys. B}. \textbf{504} pp. 345-380 (1997)
\bibitem{Catani:2015vma}Catani, S., Florian, D., Ferrera, G. \& Grazzini, M. Vector boson production at hadron colliders: transverse-momentum resummation and leptonic decay. {\em JHEP}. \textbf{12} pp. 047 (2015)
\bibitem{Ji:1996nm}Ji, X. Deeply virtual Compton scattering. {\em Phys. Rev. D}. \textbf{55} pp. 7114-7125 (1997)
\bibitem{Xie:2023xkz}Xie, G., Kou, W., Fu, Q., Ye, Z. \& Chen, X. Deeply virtual compton scattering at future electron-ion colliders. {\em Eur. Phys. J. C}. \textbf{83}, 900 (2023)
\bibitem{Favart:2015umi}Favart, L., Guidal, M., Horn, T. \& Kroll, P. Deeply Virtual Meson Production on the nucleon. {\em Eur. Phys. J. A}. \textbf{52}, 158 (2016)
\bibitem{Brooks:2018uqk}Brooks, W., Schmidt, I. \& Siddikov, M. Deeply virtual meson production on neutrons. {\em Phys. Rev. D}. \textbf{98}, 116006 (2018)
\bibitem{Kaur:2024bgo}Kaur, N. \& Dahiya, H. Transverse distortion and single-spin asymmetries for low-lying octet baryons. {\em Int. J. Mod. Phys. A}. \textbf{39}, 2450076 (2024)
\bibitem{Freese:2020mcx}Freese, A. \& Cloët, I. Quark spin and orbital angular momentum from proton generalized parton distributions. {\em Phys. Rev. C}. \textbf{103}, 045204 (2021)
\bibitem{Luan:2023lmt}Luan, X. \& Lu, Z. Generalized parton distributions of sea quark at zero skewness in the light-cone model. {\em Eur. Phys. J. C}. \textbf{83}, 504 (2023)
\bibitem{Meissner:2008ay}Meissner, S., Metz, A., Schlegel, M. \& Goeke, K. Generalized parton correlation functions for a spin-0 hadron. {\em JHEP}. \textbf{8} pp. 038 (2008)
\bibitem{Cerutti:2022lmb}Cerutti, M., Rossi, L., Venturini, S., Bacchetta, A., Bertone, V., Bissolotti, C. \& Radici, M. Extraction of pion transverse momentum distributions from Drell-Yan data. {\em Phys. Rev. D}. \textbf{107}, 014014 (2023)
\bibitem{LatticeParton:2023xdl}Chu, M. \& Others Transverse-momentum-dependent wave functions of the pion from lattice QCD. {\em Phys. Rev. D}. \textbf{109}, L091503 (2024)
\bibitem{Engelhardt:2015xja}Engelhardt, M., Hägler, P., Musch, B., Negele, J. \& Schäfer, A. Lattice QCD study of the Boer-Mulders effect in a pion. {\em Phys. Rev. D}. \textbf{93}, 054501 (2016)
\bibitem{Kou:2023ady}Kou, W., Shi, C., Chen, X. \& Jia, W. Transverse momentum dependent parton distributions of pion at leading twist. {\em Phys. Rev. D}. \textbf{108}, 036021 (2023)
\bibitem{Pasquini:2014ppa}Pasquini, B. \& Schweitzer, P. Pion transverse momentum dependent parton distributions in a light-front constituent approach, and the Boer-Mulders effect in the pion-induced Drell-Yan process. {\em Phys. Rev. D}. \textbf{90}, 014050 (2014)
\bibitem{Puhan:2023hio}Puhan, S. \& Dahiya, H. Leading twist T-even TMDs for the spin-1 heavy vector mesons. {\em Phys. Rev. D}. \textbf{109}, 034005 (2024)
\bibitem{Chen:2019lcm}Chen, J., Lin, H. \& Zhang, J. Pion generalized parton distribution from lattice QCD. {\em Nucl. Phys. B}. \textbf{952} pp. 114940 (2020)
\bibitem{Zhang:2018nsy}Zhang, J., Chen, J., Jin, L., Lin, H., Schäfer, A. \& Zhao, Y. First direct lattice-QCD calculation of the x-dependence of the pion parton distribution function. {\em Phys. Rev. D}. \textbf{100}, 034505 (2019)
\bibitem{Kaur:2018ewq}Kaur, N., Kumar, N., Mondal, C. \& Dahiya, H. Generalized Parton Distributions of Pion for Non-Zero Skewness in AdS/QCD. {\em Nucl. Phys. B}. \textbf{934} pp. 80-95 (2018)
\bibitem{AbdulKhalek:2021gbh}Abdul Khalek, R. \& Others Science Requirements and Detector Concepts for the Electron-Ion Collider: EIC Yellow Report. {\em Nucl. Phys. A}. \textbf{1026} pp. 122447 (2022)
\bibitem{Adams:2018pwt}Adams, B. \& Others Letter of Intent: A New QCD facility at the M2 beam line of the CERN SPS (COMPASS++/AMBER).  (2018,8)
\bibitem{Arifi:2024mff}Arifi, A., Happ, L., Ohno, S. \& Oka, M. Structure of heavy mesons in the light-front quark model. {\em Phys. Rev. D}. \textbf{110}, 014020 (2024)
\bibitem{Weber:1992ww}Weber, H. Light cone quark model with spin force for the nucleon and Delta (1232). {\em Phys. Lett. B}. \textbf{287} pp. 14-17 (1992)
\bibitem{Acharyya:2024enp}Acharyya, R., Puhan, S. \& Dahiya, H. Quark spin-orbit correlations in spin-0 and spin-1 mesons using the light-front quark model. {\em Phys. Rev. D}. \textbf{110}, 034020 (2024)
\bibitem{Xiao:2003wf}Xiao, B. \& Ma, B. Pion photon and photon pion transition form-factors in the light cone formalism. {\em Phys. Rev. D}. \textbf{68} pp. 034020 (2003)
\bibitem{Puhan:2024ckp}Puhan, S. \& Dahiya, H. Spatial and Transverse structure of Heavy B- and D-mesons. {\em PoS}. \textbf{HQL2023} pp. 089 (2024)
\bibitem{Acharyya:2024tql}Acharyya, R., Puhan, S., Kumar, N. \& Dahiya, H. Spectroscopy of excited quarkonium states in the light-front quark model.  (2024,8)

